Fluid Antenna Systems

Over the past decades, multiple antenna technologies have appeared in many different forms, most notably as multiple-input multiple-output (MIMO), to transform wireless communications for extraordinary diversity and multiplexing gains. The variety of technologies has been based on placing a number of antennas at fixed locations which dictates the fundamental limit on the achievable performance. By contrast, this paper envisages the scenario where the physical position of an antenna can be switched freely to one of the N positions over a fixed-length line space to pick up the strongest signal in the manner of traditional selection combining. We refer to this system as a fluid antenna system (FAS) for tremendous flexibility in its possible shape and position. The aim of this paper is to study the achievable performance of a single-antenna FAS system with a fixed length and N in arbitrarily correlated Rayleigh fading channels. Our contributions include exact and approximate closed-form expressions for the outage probability of FAS. We also derive an upper bound for the outage probability, from which it is shown that a single-antenna FAS given any arbitrarily small space can outperform an L-antenna maximum ratio combining (MRC) system if N is large enough. Our analysis also reveals the minimum required size of the FAS, and how large N is considered enough for the FAS to surpass MRC.

==> macro2.tex <==
    \newcommand{\qa}{{\bf a}}
    \newcommand{\qb}{{\bf b}}
    \newcommand{\qc}{{\bf c}}
    \newcommand{\qd}{{\bf d}}
    \newcommand{\qe}{{\bf e}}
    \newcommand{\qf}{{\bf f}}
    \newcommand{\qg}{{\bf g}}
    \newcommand{\qh}{{\bf h}}
    \newcommand{\qi}{{\bf i}}
    \newcommand{\qj}{{\bf j}}
    \newcommand{\qk}{{\bf k}}
    \newcommand{\ql}{{\bf l}}
    \newcommand{\qm}{{\bf m}}
    \newcommand{\qn}{{\bf n}}
    \newcommand{\qo}{{\bf o}}
    \newcommand{\qp}{{\bf p}}
    \newcommand{\qq}{{\bf q}}
    \newcommand{\qr}{{\bf r}}
    \newcommand{\qs}{{\bf s}}
    \newcommand{\qt}{{\bf t}}
    \newcommand{\qu}{{\bf u}}
    \newcommand{\qv}{{\bf v}}
    \newcommand{\qw}{{\bf w}}
    \newcommand{\qx}{{\bf x}}
    \newcommand{\qy}{{\bf y}}
    \newcommand{\qz}{{\bf z}}

    \newcommand{\qA}{{\bf A}}
    \newcommand{\qB}{{\bf B}}
    \newcommand{\qC}{{\bf C}}
    \newcommand{\qD}{{\bf D}}
    \newcommand{\qE}{{\bf E}}
    \newcommand{\qF}{{\bf F}}
    \newcommand{\qG}{{\bf G}}
    \newcommand{\qH}{{\bf H}}
    \newcommand{\qI}{{\bf I}}
    \newcommand{\qJ}{{\bf J}}
    \newcommand{\qK}{{\bf K}}
    \newcommand{\qL}{{\bf L}}
    \newcommand{\qM}{{\bf M}}
    \newcommand{\qN}{{\bf N}}
    \newcommand{\qO}{{\bf O}}
    \newcommand{\qP}{{\bf P}}
    \newcommand{\qQ}{{\bf Q}}
    \newcommand{\qR}{{\bf R}}
    \newcommand{\qS}{{\bf S}}
    \newcommand{\qT}{{\bf T}}
    \newcommand{\qU}{{\bf U}}
    \newcommand{\qV}{{\bf V}}
    \newcommand{\qW}{{\bf W}}
    \newcommand{\qX}{{\bf X}}
    \newcommand{\qY}{{\bf Y}}
    \newcommand{\qZ}{{\bf Z}}
    \newcommand{\qzero}{{\bf 0}}
    \newcommand{\qdh}{\triangle\qh}
    \newcommand{\qhh}{\hat\qh}
     \newcommand{\qhG}{\hat\qG}
    \newcommand{\qdH}{\triangle\qH}
    \newcommand{\qdG}{\triangle\qG}
    \newcommand{\qhH}{\hat\qH}

    \newcommand{\qdF}{\triangle\qF}
    \newcommand{\qhF}{\hat\qF}
    \newcommand{\qbh}{\bar\qh}
    \newcommand{\qbn}{\bar\qn}

    \newcommand{\tr}{\mbox{trace}}
    \newcommand{\st}{\mbox{s.t.}}
  \renewcommand{\vec}{\mbox{vec}}
    \def\bm#1{\mbox{\boldmath $#1$}}


    \newcommand{\be}{\begin{equation}} \newcommand{\ee}{\end{equation}}
    \newcommand{\bea}{\begin{eqnarray}} \newcommand{\eea}{\end{eqnarray}}
    \newcommand{\benum}{\begin{enumerate}} \newcommand{\eenum}{\end{enumerate}}
    \def\proof{\noindent\hspace{2em}{\itshape Proof : }}
    \def\aproof{\noindent\hspace{2em}{\itshape Alternative Proof : }}
    \def\endproof{\hspace*{\fill}~$\square$\par\endtrivlist\unskip}
    \def\endaproof{\hspace*{\fill}~$\square$\par\endtrivlist\unskip}

  \newtheorem{theorem}{Theorem}
  %\renewcommand{\thetheorem}{\thechapter.\arabic{theorem}}%
  \newtheorem{conjecture}{Conjecture}
  %\renewcommand{\theconjecture}{\thechapter.\arabic{conjecture}}%
  \newtheorem{definition}{Definition}
  \newtheorem{example}{Example}
  \newtheorem{lemma}{Lemma}
  \newtheorem{corollary}{Corollary}
  \newtheorem{proposition}{Proposition}
  %\renewcommand{\thelemma}{\thechapter.\arabic{lemma}}%

  \def \veclen {0.8}
  \def \uppos{1.2}
  \def \lowpos{-1.5}
  \def \recwid{0.6}
  \def \rechig{0.4}
  \def \crad{0.25}

  \def \Fwid{0.8}

  \newcommand{\tbox}[1]{%

     \bsegment
      \realmult {\rechig}{0.5} \ta
      \realmult {\recwid}{0.5} \tb
       \lvec (0 \ta)    \lvec ({\recwid} \ta)
       \lvec ({\recwid} -\ta) \lvec (0 -\ta)\lvec (0 0)
       \textref h:C v:C \htext ({\tb} 0){#1}
       \savepos ({\recwid} 0)(*ex *ey)
     \esegment
     \move (*ex *ey)}

  \newcommand{\tcir}[1]{%
     \bsegment
     \realmult {\crad}{2} \ta
       \move({\crad} 0)
       \lcir r:{\crad}
       \textref h:C v:C \htext ({\crad} 0) {#1}
       \savepos ({\ta} 0)(*ex *ey)
     \esegment
     \move (*ex *ey)}


  \newcommand{\tupnoisec}[1]{%
     \bsegment
     \realadd{\crad}{0.35}\arrowlen
     \realadd{\arrowlen}{0.08}\txtpos
     \rmove({-\crad} \arrowlen) \avec({-\crad} \crad)
     \textref h:C v:C \htext ({-\crad} \txtpos){#1}
     \esegment}

